Bursts of Activity: Temporal Patterns of Help-Seeking and Support in Online Mental Health Forums

Recent years have seen a rise in social media platforms that provide peer-to-peer support to individuals suffering from mental distress. Studies on the impact of these platforms have focused on either short-term scales of single-post threads, or long-term changes over arbitrary period of time (months or years). While important, such arbitrary periods do not necessarily follow users' progressions through acute periods of distress. Using data from Talklife, a mental health platform, we find that user activity follows a distinct pattern of high activity periods with interleaving periods of no activity, and propose a method for identifying such bursts and breaks in activity. We then show how studying activity during bursts can provide a personalized, medium-term analysis for a key question in online mental health communities: What characteristics of user activity lead some users to find support and help, while others fall short? Using two independent outcome metrics, moments of cognitive change and self-reported changes in mood during a burst of activity, we identify two actionable features that can improve outcomes for users: persistence within bursts, and giving complex emotional support to others. Our results demonstrate the value of considering bursts as a natural unit of analysis for psychosocial change in online mental health communities.

==> MOC_analysis.tex <==
We end with a short section on behavioral changes which occur post MOC, within a burst. 

For the bursts containing a MOC, we wish to determine if users undergo a behavioral change after experiencing a MOC. In order to do this, we consider only the bursts where at least one MOC occurs. We separate the user's posts before and after the first moment of change within a burst and consider the percent of posts (original posts and replies) which are replies before and after the first MOC occurs. With respect to supportive behavior, measured as the percentage of total posts which are replies versus questions, we find a significant difference pre- and post-MOC. Table. \ref{Table:MOC}.

We find overall no significant change in support type given by the user or affective language after an MOC occurs. We do find a slight increase in the supportive behavior of users after a MOC. On average, we found that 

\begin{table}
    \centering
\begin{tabular}{|p{3.2cm}|p{1.3cm}|p{1.3cm}|p{0.7cm}|}
    \hline
      &          \textbf{Pre MOC}  & \textbf{Post MOC} & \textbf{p} \\
     \hline
    \textbf{Percent of Posts which are Replies} & 51 & 57 & 0.11\\
    \hline
    \textbf{Simple Support Given} & 0.009 & 0.018 & 1 \\
    \hline
    \textbf{Complex Support Given} & 0.19 & 0.16 & 0.95 \\
    \hline
    \textbf{Network Support Given} & 0.46 & 0.37 & 1 \\
    \hline
    \textbf{Positive Affect} & 0.22 & 0.21 & 0.7 \\
    \hline
    \textbf{Negative Affect} & 0.008 & 0.009 & 0.98 \\
    \hline
\end{tabular}
\caption{Changes in behavior pre- and post- MOC. P-value is the result from a 2-way Kolmogorov-Smirnov test with null hypothesis that both variables were pulled from the same distribution}
\label{Table:MOC}
\end{table}


==> OP_actions.tex <==


\subsection{Support Type}
We examine the affects that providing various modes of support to others has on the user (supporter). Based on  the work of Andalibi et al.,~\cite{andalibi2017SelfDisclosure}, we identify three categories of positive social support which are most relevant to the TalkLife platform. The first two categories we construct are based on the Emotional Support category identified by Andalibi et al. as the most prevalent type of social support: emotional support. 

We further break down the emotional support category into (1) Simple Emotional Support and (2) Complex Emotional Support in order to determine if complexity matters.

For Simple Emotional Support, we consider only simple phrases identified by Andalibi et al. to denote emotional support such as  "Same" "Been there" "I know how you feel". Our category of Complex Emotional Support includes the same phrases from simple support, but with additional context. For example, rather than saying "I know how you feel", a user may continue with more context: "I know how you feel. Last year, I was also ...".

Our third category is selected as a proxy for support  which may be occurring between individuals either in direct messages within TalkLife (for which we do not have data) or off of the TalkLife platform: (3) Network and Instrumental Support. This category includes phrases of instrumental and network support such as: "Others feel the same way", "DM me" and "Message me on kik".
\todo[inline]{list all the phrases in the appendix}

We find that for individuals who experience a moment of change, they are more likely to give and receive more complex emotional support, less simple emotional support, and less network and instrumental support. 


\begin{table}
    \centering \footnotesize
\begin{tabular}{|p{3cm}|p{1.6cm}|p{1.6cm}|p{0.7cm}|}
    \hline
      \textbf{Support Type} & \textbf{Positive}  & \textbf{Negative} & \textbf{p} \\
     \hline
    \textbf{Simple Given} &   0.0009  &  0.0016  & 1\\
    \hline
    \textbf{Complex Given} & 3.3e-06. & 1.5e-7  & 0.04  \\
    \hline
    \textbf{Network Given} & 3.2e-07  & 7.1e-08  & 0.99 \\
    \hline
        \textbf{Simple Received} &   0.0013  &  0.002  & 1\\
    \hline
    \textbf{Complex Received} & 0.029  & 0.019  & 00.60 \\
    \hline
    \textbf{Network Received} & 6.4e-07  & 1.5e-07 & 0.99 \\
    \hline
\end{tabular}
\caption{Mean percentages of percentage of posts receiving various types of support within bursts having a MOC (positive) and not (negative). P-value is the result of a 2-way Kolmogorov-Smirnov test with null hypothesis both positive and negative sample sets come from the same distribution.}
\label{Table:PosSocSupp}
\end{table}


\textbf{Related Discussion:} While we find that individuals who experience moments of change both give and receive fewer messages of instrumental and network support, these individuals may be having conversations off of the platform which result in a MOC for the user. However, from our almost half a million posts, network and instrumental support is present in fewer than 0.3\% of the posts. Thus we feel that if MOCs result from these interactions, their prevalence will be relatively low as to not disturb our analysis. 

% \begin{table}[b]
%     \centering
%     \rowcolor{1}{}{lightgray}
%     \begin{tabular}{c c c}
%         \textbf{Category} & \textbf{Example} & \textbf{Metric}  \\
%          Positive Social Support & "I know how you feel" & \\
%          Another line & to check colors \\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}

\subsection{LIWC Based Features}

Using the psycholinguistic lexicon, Linguistic
Inquiry and Word Count (LIWC) \cite{pennebaker2003}, we determine the proportion of affective (positive and
negative affect) keywords utilized by both the user and supporters throughout a burst, Table. \ref{table:LIWC}. These LIWC categories draw upon expressive writing literature which associates language with therapeutic symptoms. 

We find users who experience a MOC within a burst, use on average $3.5x$ more positive affective words and $22x$ fewer negative affective words. In addition, these users experiencing a MOC receive $2x$ more positive affective words within the replies to their posts from others. 

\begin{table}
    \centering
\begin{tabular}{|p{1.8cm}|p{0.75cm}|p{1cm}|p{0.75cm}|p{1cm}|p{0.7cm}|}
    \hline
    & \multicolumn{2}{|c|}{\textbf{Positive}} & \multicolumn{2}{|c|}{\textbf{Negative}} & \\
    \hline
      \textbf{LIWC} & \textbf{Mean}  & \textbf{Median} & \textbf{Mean}  & \textbf{Median} & \textbf{p} \\
     \hline
    \textbf{Pos Affect OP} &   1.3  & 0.65 &  0.36 & 0.09 & 9e-29\\
    \hline
    \textbf{Neg Affect OP} & 3.3e-06. & 0 & 1.5e-7 & 0 & 0.04  \\
    \hline
    \textbf{Pos Affect Replies} & 0.49 & 0.22 & 0.2 & 0 & 2.2e-13 \\
    \hline
        \textbf{Neg Affect Replies} &   0.0013  & 0 &  0.002 & 0 & 1\\
    \hline
\end{tabular}
\caption{Positive and negative affect scores for bursts having a MOC (positive) and not (negative). P-value is the result of a 2-way Kolmogorov-Smirnov test with null hypothesis both positive and negative sample sets come from the same distribution.}
\label{Table:LIWC}
\end{table}


==> conclusions.tex <==



%We find that on average, users take $2.69$ minutes between posts within a burst, and $9.6$ days between bursts. Utilizing a natural-language based classifier, we separate bursts into positive and negative categories based on the presence of a moment of cognitive change. We identify features correlated with positve outcomes and check robustness of these features using changes in mood. Finally, we identify two actionables which a user can take to increase the likelihood they experience a positive change in mood: persistence in posting for over 15 posts, and replying to others with complex emotional support such as stating "\textit{I know how you feel, when I am feeling the same way I...}". 



% In addition, results from future work could be utilized in a more regulated platform to help identify individuals who have potentially had a series of poor interactions with the platform and are at higher risk of mental distress. Proposed future work could seek to identify such individuals and provide targeted support from trained supporters. 




% Analysis that follows from considering bursts:
% (1) once you have a MC, how do you change
% (2) what happens between bursts?
% (3) 

% Points:

% \begin{enumerate}
%     \item Formalize the concept of bursts of activity 
%         \begin{enumerate}
%             \item need to address why is this important - for user behavior in online communities
%             \item eg: future work for "user drop off" if there are relations between the bursts
%             \item related work: understanding user behavior in online communities \& mental health communities -- has always been either long term, or very short, we are doing medium
%             \item online mental health: Koustuv's paper
%         \end{enumerate}
%         \item Defining a burst---metric for burstiness of behavior on a community, then a method to choose the right N
%         \item Data
%     \item How are bursts with MOC different from those without MOC
%     \item We can use features identified in (2) to identify user actions which result in overall higher change in mood over the burst (despite not having a MOC)
%     \item prediction-like tasks in bursts
%     \begin{enumerate}
%     \item 1. within a burst, what happens after MOC, e.g.,
%     \item 2. betweeen bursts after MOC 
%     \end{enumerate}
% \end{enumerate}

% Future work: what is the relation \textit{between} bursts? Can you use the mood change / presense of MOC in one to tell the mood of another? Are they related? How much. 
% Potential use to predict when exiting the platform is "good" (person received help) or "bad" (potentially going to a worse scenario -- eg there is a paper looking at "depression" -> "suicide" I think Koustuv wrote).

% after the main contrib, we can discuss that bursts can be used for more interesting questions eg the mc and actions pre \& post and also the future work.


% Things people might ask: 
% \begin{enumerate}
%     \item why does this matter? if you're trying to analyze online community, bursts matter. 
%     \item practical significance to a company like Talklife for why to look at bursts (user metrics, interventions for mental health)
    
% \end{enumerate}


% todo:
% \begin{enumerate}
%     \item the distribution of gap times
%     \item metric for burstiness -- how can you quantify the burstiness (like how do you say how bimodal a distribution is)
% \end{enumerate}

% chat bots -- what type of replies are useful

% which samples are signif (don't vary with N) and which are more or less a function of the sample set

